Cryptographic and Financial Fairness

A recent trend in multi-party computation is to achieve cryptographic fairness via monetary penalties, i.e. each honest player either obtains the output or receives a compensation in the form of a cryptocurrency. We pioneer another type of fairness, financial fairness, that is closer to the real-world valuation of financial transactions. Intuitively, a penalty protocol is financially fair if the net present cost of participation (the total value of cash inflows less cash outflows, weighted by the relative discount rate) is the same for all honest participants, even when some parties cheat. We formally define the notion, show several impossibility results based on game theory, and analyze the practical effects of (lack of) financial fairness if one was to run the protocols for real on Bitcoin using Bloomberg's dark pool trading. For example, we show that the ladder protocol (CRYPTO'14), and its variants (CCS'15 and CCS'16), fail to achieve financial fairness both in theory and in practice, while the penalty protocols of Kumaresan and Bentov (CCS'14) and Baum, David and Dowsley (FC'20) are financially fair. This version contains formal definitions, detailed security proofs, demos and experimental data in the appendix.

==> assumptions.tex <==
%\centering
%\footnotesize
\begin{tikzpicture}
	\tikzset{>=latex}
	
% 	\tikzstyle{thin} = [line width=0.1mm]  
% 	\tikzstyle{thick} = [line width=0.5mm]  
	
%	\node [] (SARA) at (1.5, 0) {\emph{SA+RO}};
%	\node [] (UCRANCE) at (5, 0) {UC Security (NCE*)};

	\node [] (SA) at (0.9, 1) {{\bf Sequential Composability}};
		\node [] (SA2) at (0.9, 0.6) {\CompactML
		};
	\node [] (UCRA) at (5.1,-1) {\bf Universal Composability };
		\node [] (UCRA2) at (5.1,-1.4) {\bf (Controversial Assumption*)};
		\node [] (UCRANCE2) at (5.1, -1.8) {\CompactLadder};
	\node [] (UC) at (3, 3) {{\bf Universal Composability}};
	\node [] (UC2) at (3, 2.6) {\Ladder, \LockedLadder};
		\node [] (UC3) at (3, 2.3) {\AmortizedLadder, \MultiLock};
				\node [] (UCRO) at (5.1,1.0) {\bf Universal Composability +};
				\node [] (UCRO3) at (5.1,0.7) {\bf Global Random Oracle};
		\node [] (UCRO2) at (5.1,0.3) {{\tt Insured MPC}};
	
%	\draw [thick,<-] (SARA) -- node[midway,right]{} (SA2) ;
%	\draw [thick,<-] (UCRANCE) -- node[midway,left]{} (UCRA) ;
		\draw [thick,<-] (SA) -- node[midway,right]{} (UC3) ;
			\draw [thick,<-] (UCRA) -- node[midway,left]{} (UCRO2) ;
			\draw [thick,->] (UC3) -- node[midway,left]{} (UCRO) ;
	
\end{tikzpicture}
%\end{center}

==> data/reviewer_comments.tex <==


The Reviews below are from USENIX Security 2020.

\subsection{Reviewer 1}
\noindent\textbf{Comment.} The goal of this paper is to achieve financial fairness, which (confusingly) has nothing to do with whether the penalties match the cost of misbehavior. Rather, it deals with the fact that some extant protocols use multiple rounds that occur over time, and this can produce differential costs for some players based on the discount rate (e.g., if a player borrows money). 

While this may be financially sound, the analysis seems like it probably only matters in extreme cases. And more critically: the solution might be to use alternative consensus mechanisms that don't require a multi-round ladder structure.

\noindent\textbf{Reply.} A multi-round protocol is not necessarily financially unfair, and moreover designing single-round protocols that are both cyptographically and financially fair is not a trivial task. Our \CMLMech\ protocol achieves exactly this goal, improving the efficiency of \MLMech.
\medskip

\noindent\textbf{Comment.} While this paper could use some more practical components like an actual implementation (instead of just a description of the $\FuncML$ functionality), especially considering the venue, it does provide a solution to a reasonable problem ``financial unfairness" of certain schemes. In the simple ladder protocol, for example, the requirement that one party on the most extreme end must deposit (n-1)*q while some other party only needs to deposit q could end up excluding some parties from participating in these sorts of protocols. The authors also bring up the inefficiencies in some current schemes in that these schemes require a large sum of money to be put into escrow unnecessarily.

\noindent\textbf{Reply.} We added an implementation of the $\FuncML$ functionality using smart contracts, and performed additional experiments that compare executions of the \MLMech\ and \CMLMech\ protocols in terms of GAS consumption.

\medskip

\noindent\textbf{Comment.} Other citations: some techniques have proposed to solve the fairness problem, e.g., using blockchain techniques and hardware though *not* via financial penalties. See "Fairness in an unfair world" (CCS 2017) and "delta fairness". Do these analyses apply to those systems, perhaps by analyzing the cost of blockchain forgeries?

\noindent\textbf{Reply.}
The mentioned papers are unrelated to our work since they do not involve monetary compensation, but rather achieves fairness using trusted hardware (which we don't need).

\medskip

\noindent\textbf{Comment.} This paper needs a general proofread to repair grammar and fix many typos.

\noindent\textbf{Reply.} We proofread the paper and fixed all typos.

\medskip

\noindent\textbf{Comment.} Figure 3 with complexity analysis of various schemes states CML has cost $O(\lambda)$ for script complexity when it should be $O(n \cdot \lambda)$ (at least that's what the body of the text implies in the 5.1 Efficiency section).

\noindent\textbf{Reply.} The correct value is $O(n\cdot\secpar)$. We corrected the figure.

\medskip

\noindent\textbf{Comment.} Theorem 2 isn't correct in that the statement to be proven is an if and only if where only one direction is proven (if n =1 => financially fair).  The argument for the other direction (financially fair => n=1) just claims impossibility for n < 1.

\noindent\textbf{Reply.} We changed the theorem statement.

\medskip

\noindent\textbf{Comment.} For Figure 4 it's unclear precisely how the maximum amount of deposit is defined. Is it the maximum a player i must deposit in any particular round tau or is it the maximum a player i will have deposited at round tau (where deposits come from round tau and all previous rounds)? 

\noindent\textbf{Reply.} A more clear explanation has been added in Figure 4.
\medskip

\noindent\textbf{Comment.} 	Please discuss the applicability of these results to alternative smart contract systems. Please address comments in main review.

\noindent\textbf{Reply.} We made more prominent the fact that financial fairness is a general feature of any penalty protocol running with an escrow functionality, independently of how monetary compensations are enforced (be it using Bitcoin transactions, or Ethereum smart contracts). For completeness, we have also provided an implementation of the $\FuncML$ functionality in Ethereum.

\subsection{Reviewer 2}
\noindent\textbf{Comment.} The paper's premise is valid, that the time-value of money and individual differences in risk preference and financial wherewithal should be accounted for in determining the fairness of a transaction that requires financial commitment. Basic errors in the underlying calculations raise questions about the financial soundness and overall reliability of the work.

Namely,  a substantial error in the interest rate calculations that leads the authors to overstate by more than two orders of magnitude the cost of deposit. The overnight rates referred to in table 1 are customarily listed as annualized rates (with a convention of a 360-day year), but the authors calculate interest as though they were daily interest rates. This means that when they calculate a 60-minute transaction, instead of \$36K foregone on \$1M, the loss is under \$100.  -- not nothing, but a much more bearable transaction cost.

\noindent\textbf{Reply.} Thanks for this valuable comment. We have corrected the calculation of the payment interest in the box ``Conversion of Interest Rate and Computation of Payment Interest'' (from annual rate to minute rate) in \S\ref{sec:overview}. The changes have been propagated accordingly to the analysis in \S\ref{sec:fairnessanalysis}.

\medskip

\noindent\textbf{Comment.} There are two distinct aspects to the financial fairness that could be teased apart: the general time-value of money, against market discount rates; and the specific preferences of individual participants, based on their risk-sensitivity and access to capital.

\noindent\textbf{Reply.} In our paper, we only focused on how the different penalty protocols behave in terms of their inter-temporal choices. ``The specific preferences of individual participants, based on their risk-sensitivity and access to capital'' could be integrated by changing the formula in Eq.~\eqref{eq:npv}, but that is out of scope for our paper.

\medskip

\noindent\textbf{Comment.} For the first, it could be useful to compare the mechanism of interest on escrow accounts (e.g., when a landlord holds a security deposit, many U.S. states require that money to be held in interest-bearing account, with the interest accrued to the renter's benefit). 

\noindent\textbf{Reply.} This kind of security deposits are fundamentally different than those used in penalty protocols. We now clarify this in Footnote~\vref{fn:landlord}.
%\begin{quotation}\footnotesize
%	One could argue that these deposits are comparable to security deposits, in which many US states require them to be held in interest-bearing account, with the interest accrued to the depositor's benefit. That is unfortunately not true as we are talking about Bitcoin or Ethereum-based penalty protocols: once the deposits are locked, they cannot be utilized; and therefore no possible interest accrued to the ones who deposit.
%\end{quotation}	

\medskip

\noindent\textbf{Comment.} For the second, if the protocol allowed the parties to bargain over their placement in the ordering, they might be able to minimize their overall cost.

\noindent\textbf{Reply.} This would be a totally different approach than the one we use in this paper.

	


==> data/see-saw.tex <==

%\\ If we are concerning about the order of the deposits, then the protocol must be red from the roof to the foot, and from left to right (e.g. $P_i$ deposits $kq$ coins in the escrow). For the redeem order we red in the opposite verse (from foot to roof and from right to left), e.g. $P_j$ sends his transcript (and the locking token if needed) before time $\tau_{2i-1}$, and receives $kq$ money from the escrow.
% \\\\
%\begin{tabular}{llll}


%\begin{center}\footnotesize
%	\textbf{CHAIN DEPOSITS:}\\
%		\vspace{0.2cm}
%	$ P_j \xrightarrow[\deposit,\tau_{r+1}]{\hspace*{1cm} TT_{(r,1)} \hspace*{1cm}} P_1$ (for $j \in \{2,3\})$\\
%	$ P_1 \xrightarrow[\deposit,\tau_{r+1}]{\hspace*{1cm} TT_{(r-1,3)} \hspace*{1cm}} P_j$ (for $j \in \{2,3\})$\\
%	\vspace{0.2cm}
%		\textbf{LOCKED LADDER:}\\
%			\vspace{0.2cm}
%	\textbf{ROOF}: $ P_j \xrightarrow[\deposit,\tau_{r+4}]{\hspace*{1cm} TT_{(r,3)} \hspace*{1cm}} P_3$ (for $j \in \{1,2\}$)\\
%	\hspace*{0.1cm}\textbf{LADDER}:
%	$ P_3 \xrightarrow[\deposit,\tau_{r+3}]{\hspace*{1cm} TT_{(r,2)} \land U_{3,2} \hspace*{1cm}} P_2$ (Rung Unlock)\\
%	\hspace*{0.7cm} $ P_3 \xrightarrow[2 \deposit,\tau_{r+2}]{\hspace*{1cm} TT_{(r,2)} \hspace*{1cm}} P_2$ (Rung Climb)\\
%	\hspace*{1.1cm} $ P_2 \xrightarrow[\deposit,\tau_{r+2}]{\hspace*{1cm} TT_{(r,1)} \land U_{2,3} \hspace*{1cm}} P_3$ (Rung Lock)\\
%	\hspace*{-1.8cm}\textbf{FOOT}:
%	$ P_2 \xrightarrow[\deposit,\tau_{r+1}]{\hspace*{1cm} TT_{(r,1)} \hspace*{1cm}} P_1$ 
%\end{center}

%\end{tabular}

\begin{center}\footnotesize
	\textbf{ROOF}: $ P_j \xrightarrow[q,\tau_4]{\hspace*{1cm} TT_3 \hspace*{1cm}} P_3$ (for $j \in \{1,2\}$)\\
	\hspace*{0.1cm}\textbf{LADDER}:
	$ P_3 \xrightarrow[q,\tau_3]{\hspace*{1cm} TT_2 \land U_{3,2} \hspace*{1cm}} P_2$ (Rung Unlock)\\
	\hspace*{0.7cm} $ P_3 \xrightarrow[2q,\tau_2]{\hspace*{1cm} TT_2 \hspace*{1cm}} P_2$ (Rung Climb)\\
	\hspace*{1.1cm} $ P_2 \xrightarrow[q,\tau_2]{\hspace*{1cm} TT_1 \land U_{2,3} \hspace*{1cm}} P_3$ (Rung Lock)\\
	\hspace*{-1.8cm}\textbf{FOOT}:
	$ P_2 \xrightarrow[q,\tau_1]{\hspace*{1cm} TT_1 \hspace*{1cm}} P_1$ 
\end{center}



==> data/see-saw2.tex <==
By looking at the 4-party \LLMech\ it's easier to see how the locking mechanism works. Before the protocol starts the sets of players $\{P_i,P_j\}_{i,j > 1}$ agree beforehand on a token $U_{i,j}$ needed to lock and unlock the Rung Climb transaction. 
\begin{center}\footnotesize
	\textbf{ROOF}:\\
	
	 for $j \in \{1,2,3\}$: $ P_j \xrightarrow[\deposit,\tau_6]{\hspace*{1cm} TT_3 \hspace*{1cm}} P_4$\\
	 	
		\textbf{LADDER}:\\
		\begin{framed}
		\textbf{Rung Unlock (from 4 to 4)}\\
		$ P_4 \xrightarrow[\deposit,\tau_5]{\hspace*{1cm} TT_3 \land U_{4,3} \hspace*{1cm}} P_3$ \\
						\vspace{0.1cm}
			\textbf{Rung Climb}\\
		 $ P_4 \xrightarrow[3 \deposit,\tau_5]{\hspace*{1cm} TT_3 \hspace*{1cm}} P_3$ \\
		 				\vspace{0.1cm}
	\textbf{Rung lock (from 4 to 4)}\\
				$ P_3 \xrightarrow[\deposit,\tau_4]{\hspace*{1cm} TT_2 \land U_{4,3} \hspace*{1cm}} P_4$ \\
					\end{framed}
\begin{framed}
				\textbf{Rung Unlock (from 4 to 3)}\\
		$ P_4 \xrightarrow[\deposit,\tau_3]{\hspace*{1cm} TT_2 \land U_{2,4} \hspace*{1cm}} P_2$ \
				$ P_3 \xrightarrow[\deposit,\tau_3]{\hspace*{1cm} TT_2 \land U_{2,3} \hspace*{1cm}} P_2$ \\
				\vspace{0.1cm}
				\textbf{Rung Climb}\\
		$ P_3 \xrightarrow[2 \deposit,\tau_3]{\hspace*{1cm} TT_2 \hspace*{1cm}} P_2$\\
						\vspace{0.1cm}
		\textbf{Rung lock (from 4 to 3)}\\
		$ P_2 \xrightarrow[\deposit,\tau_2]{\hspace*{1cm} TT_1 \land U_{2,4} \hspace*{1cm}} P_4$ \
				$ P_2 \xrightarrow[\deposit,\tau_2]{\hspace*{1cm} TT_1 \land U_{2,3} \hspace*{1cm}} P_3$ \\
		\end{framed}
		\textbf{FOOT}:\\
		$ P_2 \xrightarrow[\deposit,\tau_1]{\hspace*{1cm} TT_1 \hspace*{1cm}} P_1$ 
		
\end{center}


==> multilock_code.tex <==

\begin{lstlisting}[basicstyle=\tiny,language=Solidity]
contract MultiLock {
	struct Player {
		uint index;
		bytes32[] commitments, shareML;
		bool hasCommitted, hasRedeemed;
		int128 shareCML; //128 bits key (16bytes)
	}
	//Let's assume that q = n as for the lottery, so that d=q(n-1) = n(n-1)
	//parameters
	uint timeDep, timeRedeem, init,d,n;
	address payable[] addresses;
	bool compactMode, redeemPhase, end;
	mapping(address => Player) players;
	constructor(address payable[] _addresses, bool _compactMode) public {
		addresses = _addresses;
		n = addresses.length;
		d = n*(n-1);
		init = now;
		timeDep = 20;
		timeRedeem = 40;
		redeemPhase = false;
		end = false;
		compactMode = _compactMode;
	}
	function lock(bytes32[] _commitments,uint _index) public payable {
		require (now < init+timeDep && msg.sender.balance >= d && msg.value >= d && msg.sender == addresses[_index] && !players[msg.sender].hasCommitted);
		players[msg.sender].commitments = _commitments;
		players[msg.sender].index = _index;
		players[msg.sender].hasCommitted = true;
	}
	function redeem(bytes32[] _share) public {
		require(redeemPhase && now < (init+timeRedeem) && players[msg.sender].hasCommitted && !players[msg.sender].hasRedeemed && !compactMode);
		Player p = players[msg.sender];
		if (keccak256(_share) == players[msg.sender].commitments[p.index]) {
			players[msg.sender].hasRedeemed = true;
			players[msg.sender].shareML = _share;
		}
	}
	function redeemCompact(int128 _share) public {
		require(redeemPhase && now < (init+timeRedeem) && players[msg.sender].hasCommitted && !players[msg.sender].hasRedeemed && compactMode);
		Player memory p = players[msg.sender];
		if (keccak256(_share) == players[msg.sender].commitments[p.index]) {
			players[msg.sender].hasRedeemed = true;
			players[msg.sender].shareCML = _share;
		}
	}
	//functions automatically checked after a certain timestamp
	function checkCommitments() public payable {
		require(!end && !redeemPhase && now >= init+timeDep);
		for (uint i = 0; i < addresses.length; i++)
			if (!players[addresses[i]].hasCommitted) { //Check that everyone has committed
				addresses[i].transfer(d);
				end = true;
				return; //return from the function if not everyone has committed
			}	
		if (checkComEq()) redeemPhase = true; //Checks if all the array of commitments are the same
	}
	function checkRedeemed() public { //if the second timestamp has passed and some player didn't redeem, penalize the players
		require(redeemPhase && now >= init+timeRedeem && !end);
		for (uint i = 0; i < addresses.length; i++) {
		if (!players[addresses[i]].hasRedeemed) 
			penalize(addresses[i]);
		}
	}	 
}
\end{lstlisting}
%pragma solidity >=0.4.21 <0.6.0;
%	//private auxiliary functions
%function penalize(address penalized) private {	//penalize dishonest players by sending the compensation
%	for (uint j = 0; j < addresses.length; j++) 
%	if (addresses[j] != penalized) addresses[j].transfer(d/(n-1)); //give d(n-1) back to player j for each j != i
%}
%function checkComEq() private returns (bool) { 
%	for (uint i = 0; i < addresses.length; i++)
%	for (uint j = 0; j < addresses.length; j++)
%	if (keccak256(abi.encodePacked(players[addresses[i]].commitments)) != keccak256(abi.encodePacked(players[addresses[j]].commitments))) return false; //Use hashes to compare the arrays
%	return true;
%}

==> rebuttal.tex <==



\reviewer \label{rA} 

\comment\label{A:summary}
This manuscript analyses MPC protocols with fairness incentivised by financial penalties from an economical point of view, characterising whether the use of collateral payments by these protocols might make the protocol financially unfair, even though it incentives rational adversaries not to cheat. 

The issue at hand is that many previous works in fair with penalties MPC requires the parties to make a collateral deposit of a quantity of funds depending on a number of parameters, e.g. the number of rounds of communication or of parties involved in the protocol. 

Given this requirement, many previous works actually require a party to make a deposit much larger than the actual cost of executing the protocol or of the financial stakes involved in that protocol. 
Moreover, in many previous works, the parties can only retrieve their deposits long after the protocol execution is finished. 
The authors show that these issues actually give an unfair advantage for parties with vast financial resources to participate in fair with penalties MPC versus parties with limited financial resources. 

The manuscript goes on to show a new approaches to building MPC protocols with fairness based on financial penalties that is financially fair according to their definitions and presents a comprehensive survey of previous works, showing which of them achieve financial fairness among other features of these protocols.

The concept of financial fairness in this context is certainly interesting and the authors do a great job of analysing the limits of this concept as well as proposing improvements to previous work that allow for achieving financial fairness. Moreover this manuscript presents a great survey of previous works outlining not only their (lack of) financial fairness but also other important features.

\reply 
We thanks the reviewer for recognizing our contributions. Indeed, our main contribution is to provide a comprehensive survey of MPC protocol with penalties, showing which of them achieve the financial fairness property. In addition we also built an illustrative financially fair protocol meeting a trade-off between security and efficiency. In particular, it achieves a weaker flavour of security with respect of some of the known works, but enhanced efficiency.
%\TODO{Make a summary of the contribution}

\comment\label{A:c0}
A minor editorial flaw is referencing previous works as Ladder (L), Multi-Lock(ML), Insured MPC (IMPC) and etc. without providing a citation to the paper that the acronym refers to to. It would be better to provide such citation in at least one central place, making it easy to quickly find out what papers the acronyms refer to. Probably Table I would be a good location for that. This is just an idea, not a required change.

\reply It has been updated accordingly in Table \ref{table:protocols}. %\TODO{put table reference}. 

\comment\label{A:c1}
However, there are two minor issues in the comparison with previous work that should be fixed before the manuscript is accepted for publication:

- It is claimed in Table I and Section V.A that the protocols L, AL, ML, LL, PL and CL are universally composable. This is not true because none of the papers describing these protocols claim UC security. The security model used to state and prove security of all protocols L, AL, ML, LL, PL and CL is proposed in [10], where the authors clearly state that they only use UC-style definitions but do not prove security in the UC model. In particular, the authors of [10] explicitly state the following: "We have not proven a composition theorem for our definition (although we believe our model should in
principle allow composition analogous to the UC composition theorem [27]).". Hence, the security model proposed in [10] and used for analysing the security of L, AL, ML, LL, PL and CL is not UC and is only conjectured by the authors to provide the same universal composition guarantees as UC (but not proven to do so).

\reply
%\TODO{Put a summary of what the reviewer said.}
As the reviewer pointed out, the authors of  L, AL, ML, LL, PL and CL did not formally prove the composition theorem for their MPC with coin UC model.
We agree that the composition theorem has not been formally proven. Anyway, we remark that assuming the correctness of their composition theorem, the UC proofs are carried out correctly. We added a footnote in Sec.\ref{subsec:hybrid} pointing out this fact. We report the footnote in the following:
\begin{quote}
\add{In \cite{BentovK14}, the authors did not formally prove the composition theorem of their augmented model. However, as the authors point out, in principle the UC composition theorem should be allowed analogously to  \cite{Canetti01}}.
\end{quote}

\comment\label{A:c2}
- In Section V.A it is correctly observed that the CL protocol from [13] has an important security issue that arises from using a random oracle based primitives inside an MPC computation. However, the authors have not mentioned that this issue also appears in LL [12], where this incorrect technique was first proposed. This observation should be added to Section V.A.

\reply 
We agree with the observation of the reviewer.
We added a footnote in Sec.~\ref{sec:eff_cri}. We report the footnote in the following:
\begin{quote}
    \add{The efficient instantiation of \LLMech\ \cite{kumaresan2015use} (which we did not analyzed in this work) has the same issue. The underlying statistical binding commitment scheme that will be used inside a circuit is instantiated with a random oracle. However, since statistical binding commitments can be instantiated also from standard assumptions, \LLMech\ still retains UC security.}
\end{quote}

%We agree that such incorrect technique first appeared in \cite{BentovKM17}.

%However, their main result is a protocol realizing the secure cash distribution reactive functionality using honest binding commitments. In Sec. 6 they present a more efficient construction of their protocol from an instantiation of honest binding commitments assuming the existence of a random oracle. Since honest binding commitment can be also instantiated from standard assumptions, a circuit describing such type of commitment for instantiations that are not in the random oracle model can be described inside an MPC functionality. Hence, their theorem is true in general. We remarked that the efficient version of their protocol cannot be proven secure in the random oracle model for the same reasoning of $\CLMech$.

\comment\label{A:c3}
Additional Questions:
1. Is the topic appropriate for publication in these transactions?: Excellent Match

\comment\label{A:c4}
1. Is the paper technically sound?: Yes

\comment\label{A:c5}
2. How would you rate the technical novelty of the paper?: Very Novel

Explain: This paper introduces the concept of financial fairness for cryptographic protocols that use financial punishments for incentivising honest behaviour, proves (im)possibility results regarding this new concept and does a comprehensive survey of current literature, classifying previous protocols w.r.t. their financial fairness while summarising their main features.

\reply We thank the reviewer. Indeed, financial fairness is a very novel contribution.% \TODO{WE USE THIS AGAINST R3.}

\comment\label{A:c6}

3. Is the contribution significant?: Significant
\comment\label{A:c7}

4. Is the coverage of the topic sufficiently comprehensive and balanced?: Yes
\comment\label{A:c8}

5. Rate the Bibliography: Satisfactory
\comment\label{A:c9}

1. How would you rate the overall organization of the paper?: Satisfactory
\comment\label{A:c10}

2. Are the title and abstract satisfactory?: Yes
\comment\label{A:c11}

3. Is the length of the paper appropriate? If not, recommend what should be added or eliminated.: Yes
\comment\label{A:c12}

4. Are symbols, terms, and concepts adequately defined?: Yes
\comment\label{A:c13}

5. How do you rate the English usage?: Satisfactory
%
\clearpage
\reviewer\label{rB}


\comment\label{B:summary}
Summary:
The paper deals with fairness in multiparty computation (MPC). It makes
the observation that the existing notion of "cryptographic fairness" is
not enough. Cryptographic fairness guarantees that honest parties will
receive either the MPC output or some monetary compensation. The problem,
however, is that this notion does not account for the "opportunity cost",
or "cost of participation". These result from the facts that parties
have to deposit money and refund it quite later in protocol, when its
actual value will have decreased, and that different parties have to lock
different amounts of money.

\reply We thank the reviewer for the recognition. Indeed financial fairness can be a key requirement for protocols handling any form of currency.% \TODO{@Nam: check this answer please}

\comment\label{B:strengths}
Strengths:
1) I believe the problem the authors have spotted is indeed important.
2) The authors define an additional property, named "financial fairness",
which accounts for the differences in monetary value over time.
3) The authors provide an overview of existing solutions and describe
why they do or do not satisfy financial fairness.
4) The authors give an interesting analysis based on hypothetically
executing realistic transactions (from Bloomberg Tradebook) on chain.
5) I liked the background on security models and assumptions presented
on the paper.

\reply We certainly believe that financial fairness is an important property that a blockchain-based protocol shall satisfy. 
Indeed, the transaction analysys in Bitcoin and Bloomberg Tradebook supports our thesis.
%\TODO{@Nam: Please check this answer}

\comment\label{B:weaknesses}
Weaknesses:
1) It is not clear what the contributions of the paper. While the Title
and Abstract mention the fairness issues, the Introduction mentions as
contribution "criteria for evaluating penalty protocols", and the fist
two of the are Security models and assumptions, and Efficiency. In my
opinion:
a) the criteria themselves should not be claimed as contributions,
but the comparison of existing protocols under these criteria is
interesting to see.

\reply  We agree with the reviewer that the first two criteria should not be claimed as contributions.
We made slight modification to point out that the contribution is financial fairness. This is highlighted under the "our contribution" paragraph in Sec. \ref{sec:intro}. We report the changes in the text below:
\begin{quote}
As a useful guide to the extant and future literature, in this 
%Systematization of Knowledge 
paper we \begin{note}recall two traditional criteria and provide a new one\ifrebuttal\reviewnotemulti{\ref{B:c3}}\fi\end{note}
for characterizing and evaluating penalty protocols: security models and assumptions, protocol efficiency and, \begin{note}for the first time, \emph{financial fairness}, defined and motivated below.
\end{note}
\end{quote}
%\TODO{We refer to A.1}

\comment\label{B:c0} Section II should be given as background and not contribution.

\reply We agree. To highlight which is the novel contribution, we distinguished between traditional and new criteria.

\comment\label{B:c1} It should be made clear what the relation between fairness and these
criteria are, and why the authors chose to include all this analysis on trust
assumptions and efficiency, when the paper (title and abstract) are on
fairness. The title and the abstract might have to be updated accordingly.

\reply Security and efficiency are the traditional criteria used to evaluate the quality of cryptographically fair MPC protocols. As an additional criteria for evaluating this class of MPC protocols, we introduced financial fairness, that is our main contribution. 
%\TODO{THIS REVIEWER IS CONFUSED. WE NEED TO EXPLAIN CLEARER. SAY WE RECALL THE FIRST TWO CRITERIA AND THE 3RD ONE WILL BE NOVEL.}

\comment\label{B:c2} The authors claim in the Conclusion that existing algorithms either
do not achieve fairness or have high complexity. The ML protocol,
however, seems to have both (Theorem 2 and Figures 3-5).

\reply The level of security is also part of the equation. 
We added a footnote in Sec.~\ref{subsec:concr_eff}. We report the footnote in the following:
\begin{quote}
   \add{Note that $\MLMech$ has higher script complexity than $\IMPC$, but provides better security guarantees. 
$\IMPC$ is asymptotically better ($O(nm)$), but we do not have enough data to to compare it with \MLMech on concrete numbers. Moreover, its security degrades because of the RO assumption.}
\end{quote}

%\daniele{I agree that Fig. 5 is misleading. Ladder should be the best one in terms of script complexity (and also in transaction fees), but it's not what appears there.}

\comment\label{B:c3} I think the existing protocols should be presented in more depth.
Only the "Ladder" protocol is described (Section IV.A), while the rest
of them (such as the ML and IMPC protocols) are only briefly described
in Table III. However, the authors prove results about ML and IMPC (and
this is a claimed contribution), so I think they should have first been
presented.

\reply We expanded on ML in Sec.~\ref{subsec:protdesc}. IMPC can be seen as a more efficient version of ML.
The expanded text follows:
\begin{quote}
    \begin{note}From this point, the functioning of \LMech\ and \MLMech\ differs.
In \MLMech\ all the players that are willing to complete the protocol engage in the $\FuncML$ functionality. 
During the Lock Phase, each party conditionally sends (locks) the same amount of coins to $\FuncML$. Each transaction is parametrized by the values $\com_i$ for all $i \in [n]$. Each party $\party_i$ shall then reveal the opening $\rndcom_i$ together with its share $\shares_i$ to $\FuncML$ before a fixed timeout (Redeem Phase). If not done, his deposit will be redistributed to the honest parties during the Compensation Phase.

More in details, during the Lock Phase, each party $\party_i$ sends to $\FuncML$ all the commitments $\com_i$ for all $i \in [n]$ received as an output of $\tilde\func$, together with a deposit $d$. If all the players sent the same commitment values and the same deposit amount before a fixed timeout $\timeout_1$, then the functionality moves to the Redeem Phase.

During the Redeem Phase, each party $\party_i$ shall send his share $\shares_i$ together with the opening $\rndcom_i$ before a fixed timeout $\timeout_2$. If all the parties provided a pair $(\shares_i,\rndcom_i)$ that is also a valid opening of $\com_i$ (i.e. such that $\Commit(\shares_i;\rndcom_i)=\com_i$), then all the deposits are given back to their owners. Now each party can use $(\shares_1,\ldots,\shares_n)$ to compute the  output of $\func$.

If at least one party $\party_i$ did not send  $(\shares_i,\rndcom_i)$ to $\FuncML$ before $\timeout_2$, his deposit $d$ will be used to compensate the other parties during the Compensation Phase. 

The \InsuredMPC\ (\IMPC)~\cite{BaumDD18} protocol can be see as a more efficient version of \MLMech\ achieving lower script complexity.
\ifrebuttal\reviewnotemulti{\ref{B:c3}}\fi
\end{note}
\end{quote}
Moreover, we also added a brief description of \LMech\ in Table 

\comment\label{B:c4} The structure of the paper maybe does not help, because I felt like
I was reading the same things in different parts. 

\reply Please see the replies to the following comments. %\TODO{WE NEED TO SAY SOMETHING BUT WE ARE NOT GONNA CHANGE STRUCTURE. @Fabio can you check it?}

\comment\label{B:c5}
For example, the
unfairness of existing protocols is discussed in Sections IV.B, VI,
and VII: Figures 2 and 6 even seem to convey the same argument, so
maybe they should be together in the text. 

\reply Fig.2 is different from Fig. 6. Fig. 2 is to illustrate the sequence of deposit in the protocol, this is useful to understand how our the money loss at the end of the protocol depends how much and when the deposits are made. Fig.6  instead is to illustrate differences in total deposit amount. 

\comment\label{B:c6} Efficiency is analysed
in Section V.B and then again in VII.

\reply In Sec.~\ref{sec:eff_sim} we analyze asymptotic efficiency, while in Sec.~\ref{subsec:concr_eff} we analyze concrete efficiency.

\comment\label{B:c7} The authors spend quite some time arguing/proving which ideas and
directions would *not* work in turning a financially unfair protocol
into a fair one, they do not really show or hint a direction that would
solve the problem. 

\reply We would remark that financial fairness is a criteria and not a methodology. Our aim is to show the trade-off between financial fairness, efficiency and security.
Compiling or designing more efficient protocols achieving cryptographic and financial fairness might be a topic for a future work.
%We added a footnote to explain this.
%\TODO{Put as a footnote when we introduce FF}

 %As shown in the paper, due to the importance of having a financially fair protocol with an high level of security, ML is the best protocol in the case of non-reactive functionalities. To illustrate such trade-off we also show a protocol with the linear script complexity and same execution time of ML. However, such protocol degrades in security, not allowing execution on a blockchain environment. CML is still applicable in contexts in which money are handled differently, and the protocol instances can be run once at a time (i.e. sequential composition). We argue more about this on the main body.
%\daniele{To nam: please check this answer. We might decide where to put this type of argumentation if not already done before.}

\comment\label{B:c8}
There is the short subsection IV.C "An Illustrative (New)
Protocol", but it is not clear whether this is a new protocol, and
whether it achieves financial fairness while being efficient.

\reply This protocol is to show the trade-off between security and script complexity while retaining both cryptographic and financial fairness.
%Our new illustrative protocol has linear script complexity (in the number of players) and same execution time of ML. However, such protocol is secure only with sequential composition, thus not allowing execution on a blockchain environment. CML is still applicable in contexts in which money are handled differently

%(e.g. centralized institutes/banks), and protocols instances can be run sequentially. We argue more about this on the main body.
%\daniele{Nam: please check this answer.}

\comment\label{B:c9}
Smaller remarks:
1) It might be a good idea to mention some of the real-world examples
early in the paper. In the beginning it was unclear to me why the money
devaluation is important or how long a protocol execution could last.

Reply: It is a good idea, we have briefly mentioned in the Introduction
\begin{quotation}
    \begin{note}
    Indeed, as shown later in our experimental evaluation, a party could suffer up to 0.49\% loss as devaluation by locking deposit in a long protocol execution time.
    \end{note}
\end{quotation}

\comment\label{B:c10}

2) A discussion on off-chain (layer 2) solutions would be important,
since this would greatly speed up the protocols and reduce costs, and
then the money devaluation would be less important.

\reply We have added a brief disucssion in a footnote in the Introduction
\begin{quotation}
\begin{note}
Recent advances in off-chain execution such as RollUp~\cite{kalodner2018arbitrum} can indeed circumvent the efficiency issue. However, the opportunity cost upon locking the deposits into the penalty protocol on-chain when boostraping the off-chain protocol is still an issue.
\end{note}
    
\end{quotation}

\comment\label{B:c11}

3) Table I: "non-reactive" and "multistage" not defined, protocols not
defined (only appear in Table III).

\reply We added a brief description of "non-reactive" and "multistage" in Table~\ref{fig:summary} and introduce the state-of-the-art protocols in the "summary of results" paragraph in Section \ref{sec:intro}. The modified text follows:
\begin{quote}
    \add{After reviewing the main state-of-the-art penalty protocols in \S\ref{sec:protocols}, namely \Ladder~\cite{BentovK14},
\MultiLock~\cite{KumaresanB14}, \InsuredMPC~\cite{BaumDD18},  \CompactLadder~\cite{kumaresan2016improvements}, \LockedLadder~\cite{kumaresan2015use},  \AmortizedLadder~\cite{KumaresanB16},  \PlantedLadder~\cite{kumaresan2016improvements}, and \CompactPL~\cite{kumaresan2016improvements}, we do an exhausting comparison using the above criteria. Moreover, in \S\ref{subsec:newprot} we introduce a new protocol, namely \CompactML, to illustrate the trade-off that a protocol must face when financial fairness must be taken into account.
A comprehensive summary of the comparisons done throughout the paper is given in Tab.~\ref{fig:summary}.}
\end{quote}

\comment\label{B:c12}
4) Table II: What are "Median hour" and "Median Minute", and why is 
"Min" larger than "Max"?

\reply Fixed (Table~\ref{table:usdep}). 

\comment\label{B:c13}
5) Example in III.A: It seems the formula used is not exactly the one
in (1).

\reply The example in Sec.~\ref{sec:escrow_overview} has been fixed.

\comment\label{B:c14}
6) Figure 1: Symbol $d_{i,t'}$ is not defined, and the API of the methods
seems to be not the same as used in the text (page 5, lines 42, 44).

\reply We updated the APIs in Sec.~\ref{sec:fescrow} accordingly, add defined the symbol the $d_{i,t'}$ in Fig. \ref{fig:escrow} . 

\comment\label{B:c15}
7) Section IV.B: "Rounds" are mentioned, but the diagram in IV.A does
not mention rounds.

\reply Prot. Steps and rounds are the same. In Fig.~\ref{fig:ladder4} we changed it to \#Rounds to avoid confusion.

\comment\label{B:c16}

8) Formula (1) is given with $\eta_{i}$, i.e., different for each party,
but a global $\eta$ is then used. Is it even possible to define fairness
if each party can define their own discount rate? If yes, should the paper
do it?

\reply We have clarified in a footnote that
\begin{quotation}
    \begin{note}
    Our model is agnostic to the rates of the parties. We use a global $\eta$ for sake of simplicity. Furthermore, most economic models assume market conditions in equilibrium as otherwise arbitration will happen. Indeed, the parties might have different utility functions and one can generalize it but it is immaterial for our discussion as we focus on the opportunity cost upon locking deposits. Some specific users might be risk averse, others on the other hand might be myiopic and it is unknown to the protocol designer. As such one cannot base a design on the assumption that the protocol only works if there is a risk-seeker participant or else.
    \end{note}
\end{quotation}


\comment\label{B:c17}

9) Section VII: Why is the "55 transactions per day" in Bloomberg
translated to "55 parties in a protocol" in the benchmark?

\reply As we have anonymous data we assume for the worst case that 55 transactions per day is interpreted as 55 parties.

\comment\label{B:c18}
10) Section VIII: It is a bit unclear what this section adds to
the results before it, and why it is called "playing it for real".
Were the previous examples not based on real data?

\reply The previous results are toy example with only 4 parties and the Bloomberg/Bitcoin example is with empirical data.

\comment\label{B:c19}

11) Reference for ML is sometimes [10] sometimes [11].

\reply Corrected. ML is \cite{KumaresanB14} now.

\comment\label{B:c20}

12) Reference [28].

\reply Corrected.

\comment\label{B:c21} 
Typos:
\begin{itemize}
    \item Many cases of fullstop without empty space after it, e.g.,
(page.line.column) 3.49.2, 4.28.1, 4.55.2, 6.28.2, 7.50.2, 10.56.1
\item "an concern", "made whole" (what does it mean here?), "criteria \#1"
(criterion 1), "wee", "on such assumption", "e.g", "worth the bother",
"using", "call unfair play" (what do we mean), missing "Sec" in 8.19.1,
"a mall collateral", "the goal of designing" (the goal is designing,
probably).
\end{itemize}


\reply All the listed errors have been fixed.

\comment\label{B:c22}
Additional Questions:
1. Is the topic appropriate for publication in these transactions?: Excellent Match

\comment\label{B:c23}

1. Is the paper technically sound?: Yes

\comment\label{B:c24}

2. How would you rate the technical novelty of the paper?: Novel Enough for Publication

\reply We agree that our paper is technically novel, and of enough novelty to be published.

\comment\label{B:c25}
Explain: The authors present a new fairness property for MPC
protocols, one that overcomes previous fairness
limitations. They examine existing protocols based on
this property and prove which ones satisfy it.
Although I think this is already enough, the authors do
not give sufficient guidelines (or new protocols)
on how to achieve that property.

\reply Thanks for your comment. Indeed, we focus on introducing an evaluation criteria and not a methodology (i.e. give further guidelines) as itself could be the topic of a paper.

\comment\label{B:c26}
3. Is the contribution significant?: Moderately Significant

\comment\label{B:c27}
4. Is the coverage of the topic sufficiently comprehensive and balanced?: Treatment somewhat unbalanced, but not seriously so

\comment\label{B:c28}
5. Rate the Bibliography: Satisfactory

\comment\label{B:c29}
1. How would you rate the overall organization of the paper?: Poor

\comment\label{B:c30}
2. Are the title and abstract satisfactory?: Yes

\comment\label{B:c31}
3. Is the length of the paper appropriate? If not, recommend what should be added or eliminated.: No (Explain):

\comment\label{B:c32}
4. Are symbols, terms, and concepts adequately defined?: Yes

\comment\label{B:c33}
5. How do you rate the English usage?: Satisfactory

\clearpage
\reviewer\label{rC}

\comment\label{C:summary}

[+]  The authors make the first steps in analysing economic aspects of secure MPC protocols known from the literature. If done properly, this may have an impact on the economy/industry;

[+]  The authors use time-discounting on deposits paid by the participants in MPC. This allows a better understanding of the incentives of the users;

[+]  The authors refer to practical examples such as BitCoin, and Bloomberg Tradebook. Even though the examples are hardly generalizable, they serve as an indication of the authors’ involvement in the world of finances. This may help authors to develop efficient solutions in the future.

\reply Thanks for recognizing our contribution. For the Bitcoin/Blommberg example, we use them as illustration as they are the most popular instruments in the real world. Indeed, Financial Fairness is an evaluation criteria, not a methodology. Thus we are not looking into improvements of penalty protocols.

\comment\label{C:disadvantages}
Disadvantages

[-]  My main concern is about the following: academic novelty, quality and impact of the research are insufficient for journal publication. The authors compare already existing MPC protocols without any attempt to develop new concepts and/or solutions. 

\reply With respect to academic novelty,
both reviewer A (see \ref{A:c5}) and reviewer B  (see \ref{B:c24}) agree that we have made sufficient contribution and that our work is novel enough for publication.
Furthermore we have improved the quality  of the paper as we addressed the reviewers' comments (see e.g. \ref{A:c1}, \ref{A:c2},\ref{B:weaknesses},\ref{B:c3}, \ref{B:c11}). For instance, we have added argumentation about the importance of considering financial fairness in the industrial setting. In fact, Bitcoin is a the most popular decentralized network and Bloomberg Tradebook is a practical industrial application where security is essential (as cryptographic and financial fairness are both important: who would use a protocol that one can scott-free abort or one has to pay more to achieve the same purpose).
Indeed, our purpose is to introduce a whole new dimension that has not been considered before in MPC protocol. This also acknowledged by Reviewer A and Reviewer B (see for example \ref{A:summary}, \ref{B:summary},\ref{B:strengths}).

\comment\label{C:c0}
In addition, the possible impact of such a comparison is not explained by the authors. How can the conclusions of the paper help the average user who is willing to participate in MPC? Can authors guide developers of corresponding MPC platforms? How can these findings be useful for the economy/industry?

\reply We argue that the lack of attention to financial aspects is also one of the causes behind lack of adoption. The focus is at first on designers. Users can use the model and the software we have used for simulations and our software to check whether the protocol meets their interests. Guide on developers we have used the “illustrative protocol” to guide designers into the alternative choices. We added a paragraph on implications for practice in the main text. See the reply to \ref{C:disadvantages} and the paragraph "Implication or Practice" in Section \ref{sec:intro}.

\comment\label{C:c1}
[-]  The severity of the former comment is amplified due to the absence of a Research Question (RQ). Partially because of this, the paper lacks guidance: for instance, it remains unclear how section ‘II. SECURITY AND EFFICIENCY’ contributes to answering such an obscure RQ.

\reply This is indeed a very good point, we have taken the advice and casted the problems as RQs to clarify the contribution.
The RQ has been added in Section \ref{sec:intro}.

\comment\label{C:c2}
[-]  The authors introduce a new but unnecessary definition of ‘financial fairness’. 

\reply See reply to comment \ref{C:disadvantages} and comments \ref{A:summary} and \ref{B:summary}.

\comment\label{C:c3}
To communicate the importance of their work, the authors use vague argumentation such as ‘…we believe that the outcome’s valuation should be at least fair from the viewpoint of a protocol designer…’ (p. 4, right column, line 50). In that regard, the authors should be reminded that IEEE T-IFS is NOT The Journal of Theological Studies (https://academic.oup.com/jts), and their beliefs are not of the major concern of the journal audience. 

\reply We have removed the offending sentence, but the paper shows several different scientific argumentation on why the definition is important, including theoretical results of importance to designers (Section \ref{sec:thfin}) and practical simulations (Section \ref{sec:concsim}).%\TODO{Remove the sentence. Adjust}

\comment\label{C:c4}
Regrettably, such argumentation is provided without any effort to connect the so-called ‘financial fairness’ with the already existing body of knowledge including Expected Utility Theory (EUT) and Mean-Variance (M-V) analysis. On the one hand, ‘financial fairness’ analysed by the authors is tightly connected with the wealth variance which is the well-known part of the M-V. On the other hand, the paper suffers from impaired reasoning about the MEAN OF THE WEALTH that is acquired by the participants in different MPC protocols.

\reply Please see reply \ref{C:c0}.

%$\sum_t U(x_t,t)$ our particular example is $U(x_t,t) = x_t * e^{-rt}$. We can add a paragraph on UT. 
%Utility theory is relevant as there might different functions to evaluate the temporal dimension of the amount of money that is deposited (for example prospect theory)
%Expected Utility Theory and Mean-Variance analysis are not relevant as they have to do with a portfolio evaluation in presence of (typically) stochastic uncertainty of returns. 
%For example one uses MV or EUT to establish that an investment in assets X is “better” than an investment in assets Y because X might return 10% of the initial investments and do so with very low volatility (i.e. variance) while Y might return 20% but do so with a very high volatility or even generate a loss. Depending on the risk aversion of the user,  A and B might therefore be better than X and Y.
%Here there is no stochastic uncertainty in the returns of the deposits or the withdrawals are entirely deterministic. There is only an epistemic uncertainty as a player might decide to stop the protocol beforehand
%The only possible stochastic uncertainty is the final evaluation of the overall ‘outerprotcol” if such outcome have elements of stochastic uncertainty (e.g. the result of the actual poker hand). However this is immaterial to the penalty protocol to arrive to the final state.\\
%Actor A = $\sum_t U_A(x_t,t) + U_A$ (final state for A for the outer protocol)\\
%Actor B = $\sum_t U_B(x_t,t) + U_B$ (final state for B for the outer protocol)\\
%We generalize the section on the Utility to use a utility function and use the exponential discount with risk neutral evaluation as an example for the calculation

\comment\label{C:c5}
[-]  The authors make an implicit (and unjustifiable) assumption about the economic aspects of MPC protocols. For example, it is erroneously assumed that the valuations for coins/tokens (for security deposits and rewards) in different protocols are equal: the same variable $q$ (page 8) is used to express the nominal value of the coin in L and ML protocols. Without clarifying these valuations, it is impossible to discuss utilities in different protocols! 

\reply We believe there is a misunderstanding here. From a technical perspective all participants to a protocol are bound to it, otherwise it is technically impossible. We do not discuss utilities across different protocols, but utilities within runs of the same protocol. The same apply to crypto-fairness which is a property of a protocol. Please see the "Implications for Practice" paragraph in Section \ref{sec:intro}.
%\TODO{Add pointer: implication for practice.}

\comment\label{C:c6}
The mentioned valuations are, however, subject to the factors affecting parties who opt for one or the other protocol. The latter should be studied in both socio-economical (e.g. mutual trust within the participants, their risk appetites, the popularity of specific MPC protocol, market anticipations for the price of coins/tokens used by each MPC protocol, how early in time the protocol was introduced to the public, etc.) and technical (e.g. validity of assumptions, requirements to the software/hardware running MPC protocol, usability etc.) domains. 

\reply Indeed one could introduce further complications into the model, especially from the socio-economical aspects. We borrowed the text of the reviewer and leave the further complications as future work.

%This is a very question interesting on why one should run something but it is immaterial to the present discussion. What kind of MPC protocols could be practically deployed depends on a wealth of questions (including the existence of software libraries). However we are focusing here on the properties of each individual protocol. We put it into the section implication.\TODO{@Nam}

\comment\label{C:c7}
There are many examples (e.g. among cryptocurrencies) where for some consensus protocols miners’ rewards have higher variance, but the stakes (and rewards) are larger, too – due to historical, social or technological reasons. Hence, the premise for protocol comparison should be this: “If the nominal of deposit/reward coin is the same for all protocols (explain why it must be the case)… then a rational participant should select protocol X because its expected utility is the highest”. 

\reply Please see the "Implications for Practice" paragraph in Section \ref{sec:intro}.
%We are NOT comparing rewards of different protocols so we are not comparing participant 1 using protocol A and participant B using protocol 2, because they can NOT do it. All participants in a protocol do have the same protocol! A protocol must be agreed by all participants and therefore it must be fair for all participants. 
%The discussion on the final rewards is very relevant for the final state of B or the final state for A (or the initial states) but this is immaterial to the individual protocol chosen.

\comment\label{C:c8}
Valuations of deposit coins in different MPC protocols may also affect the incentives of participating parties to abort executions at different moments. Consequently, the probabilities of such abortions will affect the expected utilities of participants. This aspect has been largely ignored by the authors: the construct of Theorem 4 is clearly insufficient for such analysis.

\reply Thanks. This is yet another good consideration for the full scenario. We have added this as a possible future work into the paper at the end of Section \ref{subsec:openproblems}. We also report the new paragraph in the following:
\begin{quote}
    \begin{note}
\emph{Compiling unfair protocols into fair ones.}
A natural open question is whether a financially unfair protocol like \LMech\ can be compiled into a fair protocol while keeping comparable efficiency and security. 
\end{note}
\end{quote}

\comment\label{C:c9}
[-]  The limit on the number of parallel protocol runs remains unclear. The authors implicitly suggest that one protocol instantiation can be run at a time. Is it really the case? This is especially troubling taking into account the attention authors pay to time discounting: parallel runs increase the speed of wealth accumulation. For instance, if for all protocols the complexity of locally computed share is negligible, and the tasks are in abundance (an infinite number of tasks can be run in parallel) then all the considered MPC protocols are equally attractive. I can only provide the following suggestion: the number of parallel runs may be constrained by the funds (for deposits) available to each participant. Several additional (but justifiable!) assumptions must be done in that regard.

\reply You must be referring to the Illustrative protocol. This is used as an example of the trade-off between economic and security. It cannot be run in parallel as otherwise it will be insecure. We have added further explanation on this case (in the paragraph "Further considerations" in Section \ref{subsec:newprot}):
\begin{quote}
\add{Note that if the complexity of locally computed share is negligible, and the tasks are in abundance (an infinite number of tasks can be run in parallel) then all financially fair MPC protocols would be equally attractive as they might  be constrained by the funds (for deposits) available to each participant. However, running our illustrative protocol might become insecure and thus vulnerable to attacks violating cryptographic fairness or the privacy of the parties' inputs.}
\end{quote}

\comment\label{C:c10}
[-]  The authors appeal to special cases (e.g. BitCoin, Bloomberg Tradebook) to argue about the execution time of the protocols. However, they do this without proper justification. This is unacceptable: specific timing determines absolute differences between expected utilities in different protocols. While the protocol preference order may not change (provide proof, please), the argumentation becomes weaker when time-discounting diminishes. Hence, justification should be in this form: ‘Bloomberg Tradebook and BitCoin are the ONLY possible means to execute MPC protocols because…’.

\reply Please see the "Implications for Practice" paragraph in Section \ref{sec:intro}.

%We are not not sure we understood the claim of the reviewer. We never claimed that Bloomerg or Bitcoin are the only possible means. We show that IF one use these data, the effects will be the one shown in the paper. We borrowed the text of reviewer to say that 
%This is an illustrative example, specific timing determines absolute differences between expected utilities in different protocols. While the protocol preference order may not change when time-discounting varies, the effect might also vary. We chose those because Bitcoin is a the most popular decentralize network and Bloomberg because it is a practical industrial application where security is essential or whatever

\comment\label{C:c11}
[-]  There are numerous inconsistencies in the paper:

a) Abbreviations PPT and RO first appear on pp. 2 and 3, respectively, without any clarification;

\reply We expanded the acronyms.

\comment\label{C:c12}
b) On p.5, left column, line 19 ‘…fairness grounded in the economic literature’. The authors clearly ignored many relevant sources dealing with EUT and M-V;

\reply Please see our answer in \ref{C:c4}.

\comment\label{C:c13}
c) On p.5, right column, line 20, Definition 1. The authors require $\chi_{i} = \chi_{j}$ while expected utilities should be used instead: $\mathbb{E}\left(\mathcal{U}_i \right) = \mathbb{E}\left(\mathcal{U}_j \right)$;

\reply Please see our answer in \ref{C:c4}. %We are not working with EUT but with the NPV.

\comment\label{C:c14}
d) On p.9, left column, line 21 ‘…final large reward with certainty.’ There is no such thing as ‘certainty’. Instead, there is an expectation;

\reply Please see our answer in \ref{C:c4}.

\comment\label{C:c15}
e) Expression for $\chi_{55} (110)$ on p. 10, right column, line 35 is incorrect: the power of the exponent should be negative;

\reply Thanks for noticing and pointing this out. Indeed the exponent should be negative. All the values have been recalculated.
%\TODO{@Nam: please double check. I changed put the negative and recalculated everything. The old text is commented.}

\comment\label{C:c16}

f) On p. 11, right column, multiple appearances in the text. The authors refer to the ‘worst case’. There must be a justification (e.g. a proof) that this is the worst case in expectation (involving many runs of the protocol);

\reply We explained it in a footnote near the first appearence of "worst case party" in Section \ref{sec:comparisons}.

\comment\label{C:c17}

g) Phrase “…from 47 minutes to 75 minutes on average” (p. 12, right column, line 6) is unclear: ‘on average’ should be a scalar value and not the range;

\reply We agree that it is a scalar value. We removed "on average".

\comment\label{C:c18}

h) On p. 12, right column, line 3, the authors write “We make no assumption on the function used to compute the net present value,…” which is confusing since they explicitly suggest exponential discounting on p.10, for example;

\reply We use exponential discounting only for illustration purposed. We explained it in a footnote in the "Relation to Expected Utility Theory" paragraph of Section \ref{sec:intro}.

\comment\label{C:c19}

[-]  A unified table of mathematical symbols for the whole paper would be helpful.

\reply A unified table of mathematical symbols has been provided in Table \ref{tab:symbols}.

\comment\label{C:c20}

Additional Questions:
1. Is the topic appropriate for publication in these transactions?: Adequate Match

\comment\label{C:c21}
1. Is the paper technically sound?: No

\comment\label{C:c22}
2. How would you rate the technical novelty of the paper?: Not Novel
Explain: The authors attempt to develop an intuitive concept about the fairness of the penalty protocols in secure Multi-Party Computations (MPCs). They stipulate fairness as the condition where the net present cost of participation (the total value of cash inflows less cash outflows, weighted by the relative discount rate) is the same for all honest participants, even when some parties cheat. The authors claim that the ladder protocol (CRYPTO’14), and its variants (CCS’15 and CCS’16), fail to achieve financial fairness both in theory and in practice, while the penalty protocols of Kumaresan and Bentov (CCS’14) and Baum, David and Dowsley (FC’20) are financially fair.

\reply As also recognized by the reviewer C, our contribution is the proposal and definition of Financial Fairness and the analysys of existing protocols using the new metric. Reviewer A and B recognize the same and acknowledge the technical novelty of our paper and agree that such a contribution is sufficient for publication, please see comments \ref{A:summary},\ref{A:c5},\ref{B:summary}, \ref{B:strengths} and \ref{B:c24}.

\comment\label{C:c24}
My main concern is about the following: academic novelty, quality and impact of the research are insufficient for journal publication. The authors compare already existing MPC protocols without any attempt to develop new concepts and/or solutions. In addition, the possible impact of such a comparison is not explained by the authors. How can the conclusions of the paper help the average user who is willing to participate in MPC? Can authors guide developers of corresponding MPC platforms? How can these findings be useful for the economy/industry?

\reply Both reviewer A (in \ref{A:c5}) and reviewer B  (in \ref{B:c24}) agreed that we made sufficient contribution and that our work is novel enough for publication.
We improved the quality  of the paper (see e.g. \ref{A:c1}, \ref{A:c2},\ref{B:weaknesses},\ref{B:c3}, \ref{B:c11}). In particular, we added some argumentation about the importance of considering financial fairness in the industrial setting. In fact, Bitcoin is a the most popular decentralized network and Bloomberg is a practical industrial application where security is essential (as cryptographic and financial fairness are both important: who would use a protocol that one can scott-free abort or one has to pay more to achieve the same purpose).
Our purpose is to introduce a whole new dimension that was never thought before applicable to MPC protocol. This also acknowledged by Reviewer A and Reviewer B (\ref{A:summary}, \ref{B:summary},\ref{B:strengths}). 
We would remark that financial fairness is a criteria and not a methodology. Our aim is to show the trade-off between financial fairness, efficiency and security. We are not giving guidelines.
Compiling or designing more efficient protocols achieving cryptographic and financial fairness might be a topic for a future work.


\comment\label{C:c25}

3. Is the contribution significant?: Incremental

\comment\label{C:c26}

4. Is the coverage of the topic sufficiently comprehensive and balanced?: Important Information is missing or superficially treated

\comment\label{C:c27}

5. Rate the Bibliography: Unsatisfactory

\comment\label{C:c28}

1. How would you rate the overall organization of the paper?: Could be improved

\comment\label{C:c29}

2. Are the title and abstract satisfactory?: Yes

\comment\label{C:c30}

3. Is the length of the paper appropriate? If not, recommend what should be added or eliminated.: Yes

\comment\label{C:c31}

4. Are symbols, terms, and concepts adequately defined?: Not always

\comment\label{C:c32}

5. How do you rate the English usage?: Needs improvement



\clearpage
\twocolumn
\setcounter{page}{1}

==> see-saw2.tex <==
By looking at the 4-party \LLMech\ it's easier to see how the locking mechanism works. Before the protocol starts the sets of players $\{P_i,P_j\}_{i,j > 1}$ agree beforehand on a token $U_{i,j}$ needed to lock and unlock the Rung Climb transaction. 
\begin{center}\footnotesize
	\textbf{ROOF}:\\
	
	 for $j \in \{1,2,3\}$: $ P_j \xrightarrow[\deposit,\tau_6]{\hspace*{1cm} TT_3 \hspace*{1cm}} P_4$\\
	 	
		\textbf{LADDER}:\\
		\begin{framed}
		\textbf{Rung Unlock (from 4 to 4)}\\
		$ P_4 \xrightarrow[\deposit,\tau_5]{\hspace*{1cm} TT_3 \land U_{4,3} \hspace*{1cm}} P_3$ \\
						\vspace{0.1cm}
			\textbf{Rung Climb}\\
		 $ P_4 \xrightarrow[3 \deposit,\tau_5]{\hspace*{1cm} TT_3 \hspace*{1cm}} P_3$ \\
		 				\vspace{0.1cm}
	\textbf{Rung lock (from 4 to 4)}\\
				$ P_3 \xrightarrow[\deposit,\tau_4]{\hspace*{1cm} TT_2 \land U_{4,3} \hspace*{1cm}} P_4$ \\
					\end{framed}
\begin{framed}
				\textbf{Rung Unlock (from 4 to 3)}\\
		$ P_4 \xrightarrow[\deposit,\tau_3]{\hspace*{1cm} TT_2 \land U_{2,4} \hspace*{1cm}} P_2$ \
				$ P_3 \xrightarrow[\deposit,\tau_3]{\hspace*{1cm} TT_2 \land U_{2,3} \hspace*{1cm}} P_2$ \\
				\vspace{0.1cm}
				\textbf{Rung Climb}\\
		$ P_3 \xrightarrow[2 \deposit,\tau_3]{\hspace*{1cm} TT_2 \hspace*{1cm}} P_2$\\
						\vspace{0.1cm}
		\textbf{Rung lock (from 4 to 3)}\\
		$ P_2 \xrightarrow[\deposit,\tau_2]{\hspace*{1cm} TT_1 \land U_{2,4} \hspace*{1cm}} P_4$ \
				$ P_2 \xrightarrow[\deposit,\tau_2]{\hspace*{1cm} TT_1 \land U_{2,3} \hspace*{1cm}} P_3$ \\
		\end{framed}
		\textbf{FOOT}:\\
		$ P_2 \xrightarrow[\deposit,\tau_1]{\hspace*{1cm} TT_1 \hspace*{1cm}} P_1$ 
		
\end{center}

